The Space Complexity of Consensus from Swap

Nearly thirty years ago, it was shown that $\Omega(\sqrt{n})$ registers are needed to solve obstruction-free consensus among $n$ processes. This lower bound was improved to $n$ registers in 2018, which exactly matches the best upper bound. The $\Omega(\sqrt{n})$ space complexity lower bound actually applies to a class of objects called historyless objects, which includes registers, test-and-set objects, and readable swap objects. However, every known $n$-process obstruction-free consensus algorithm from historyless objects uses $\Omega (n)$ objects. We give the first $\Omega (n)$ space complexity lower bounds on consensus algorithms for two kinds of historyless objects. First, we show that any obstruction-free consensus algorithm from swap objects uses at least $n-1$ objects. More generally, we prove that any obstruction-free $k$-set agreement algorithm from swap objects uses at least $\lceil \frac{n}{k}\rceil - 1$ objects. This is the first non-constant lower bound on the space complexity of solving $k$-set agreement with swap objects when $k > 1$. We also present an obstruction-free $k$-set agreement algorithm from $n-k$ swap objects, exactly matching our lower bound when $k=1$. Second, we show that any obstruction-free binary consensus algorithm from readable swap objects with domain size $b$ uses at least $\frac{n-2}{3b+1}$ objects. Since any historyless object can be simulated by a readable swap object with the same domain, our results imply that any obstruction-free consensus algorithm from historyless objects with domain size $b$ uses at least $\frac{n-2}{3b+1}$ objects. For $b = 2$, we show a slightly better lower bound of $n-2$. The best known obstruction-free binary consensus algorithm from readable swap objects with domain size $2$ uses $2n-1$ objects, asymptotically matching our lower bound.

==> unreadable.tex <==
\section{Set Agreement Algorithm from Swap}\label{sec:unreadableub}

In this section, we present upper and lower bounds on the space complexity of solving nondeterministic solo-terminating $k$-set agreement from swap objects.
We emphasize that a swap object does not support the \emph{Read} operation.
For consensus (i.e. $k = 1$), our upper and lower bounds match exactly.


We begin by describing an obstruction-free, $m$-valued, $k$-set agreement algorithm from $n-k$ swap objects $B_1, \ldots, B_{n-k}$.
Every swap object stores two fields.
The \emph{lap counter} field consists of an array of $m$ values, all initially $0$, and the \emph{identifier} field consists of a single value, initially $\bot$.


We can view the algorithm as a race between the input values.
Every process $p$ stores a local lap counter $U[0,\ldots,m-1]$ that holds the highest lap for each input value that has been observed by $p$.
If $U[x] > U[x']$, for some $x, x' \in \{0, \ldots, m-1\}$, then $p$ believes that the value $x$ is ahead of the value $x'$ in the race.
Each process $p$ maintains a preference $v$ equal to the value that $p$ believes is leading the race.
That is, $U[v] \geq U[j]$, for all $j \in \{0, \ldots, m-1\}$.
Initially, the preference of process $p$ is equal to its input value.
During the algorithm, process $p$ repeatedly attempts to complete a lap for its current preference $v$.
To complete a lap, process $p$ must observe its own process identifier in the identifier field of every object.
When $p$ sees that its preference $v$ is sufficiently far ahead of all the other values, it decides the value $v$.

%\setlength{\textfloatsep}{6pt}

\begin{algorithm2e}
\caption{An obstruction-free, $m$-valued, $k$-set agreement algorithm from $n-k$ swap objects.}
\label{alg:consswap}

\setstretch{1}

\SetKwProg{Fn}{Function}{:}{}
	\DontPrintSemicolon
	\SetKwFor{Loop}{loop}{}{end}
	
	\nonl\textbf{shared:} swap objects $B_1, \ldots, B_{n-1}$, initially $B_1 = \ldots = B_{n-k} = \bigl\langle [0, \ldots, 0], \bot \bigr\rangle$\;
	\Fn{$propose(v)$ by process $p$}{
		$U[0, \ldots, m-1] \gets [0, \ldots, 0]$\;\label{ln:init1}
		$U[v] \gets 1$\;\label{ln:init2}
		\Loop{}{\label{ln:mainloop}
			$\textit{conflict} \gets \textsc{False}$\;
			\For{$i \in \{1, \ldots, n-k\}$}{\label{ln:swaploop}
				$\langle U', p'\rangle \gets Swap(B_i, \langle U, p\rangle)$\;
				\If{$\langle U', p'\rangle \neq \langle U, p\rangle$}{
					$\textit{conflict} \gets \textsc{True}$\;
					\For{all $j \in \{0, \ldots, m-1\}$} {\label{ln:updatelocal}
						$U[j] \gets$ max$\bigl(U[j], U'[j]\bigr)$\;\label{ln:setmaxlocal}
					}
					$c \gets$ max$(U)$\;\label{ln:maxval}
					$v \gets$ min$\bigl\{j\; :\; U[j] = c\bigr\}$\;\label{ln:minindex}
				}
			}
			\If{$\textit{conflict} = \textsc{False}$}{\label{ln:conflictcond}
				\If{for all $j \neq v$, $U[v] \geq U[j] + 2$}{\label{ln:decidecond}
					\textbf{decide} $v$\;\label{ln:decide}
				}
				\Else{
					$U[v] \gets U[v] + 1$\;\label{ln:inc}
				}
			}
		}
		
	}
\end{algorithm2e}



Algorithm~\ref{alg:consswap} is a pseudocode description of our algorithm.
A process $p$ with input $v$ begins by initializing its local lap counter $U$ such that $U[j] = 0$ for all $j \in \{0, \ldots, m-1\} - \{v\}$, and $U[v] = 1$.
Process $p$ then begins the loop on line~\ref{ln:mainloop}, which we will call the main loop.
An iteration of the main loop begins with $p$ entering the inner loop on line~\ref{ln:inloop}.
During the inner loop, $p$ swaps the pair $\langle U, v\rangle$ into the objects $B_1, \ldots, B_{n-1}$ one at a time.
If $p$ sees another process' identifier in the response to one of these swaps, it enters the block on line~\ref{ln:idcond}.
In this block, process $p$ updates every component $j$ of its local lap counter to the maximum of $U[j]$ and $U'[j]$, where $U'$ is the lap counter that $p$ obtained from its previous swap.
Process $p$ then updates its preference $v$ to be the index of its new lap counter that has the highest lap value.
If there are multiple indices with the highest lap value, then $p$ chooses $v$ to be the smallest of these indices (lines~\ref{ln:maxval} and \ref{ln:minindex}).
Then $p$ restarts its inner loop.

If $p$ swaps all of the objects and sees its own process identifier in the response to each of these swaps, then $p$ checks whether its preference $v$ is far enough ahead of all the other values on line~\ref{ln:decidecond}.
If the value $v$ is at least $2$ laps ahead of every other value in $p$'s local lap counter $U$, then $p$ decides $v$.
Otherwise, $p$ completes a lap for $v$ by incrementing $U[v]$ on line~\ref{ln:inc}.

\medskip

If $V$ and $V'$ are two $m$-component vectors, then we say $V \preceq V'$ if and only if $V[j] \leq V'[j]$, for all $j \in \{0, \ldots, m-1\}$.
Let $\alpha$ be an execution of Algorithm~\ref{alg:consswap} from some initial configuration $C_0$.

After process $p$ initializes its local lap counter on lines~\ref{ln:init1} and \ref{ln:init2}, we know that $U[v]$ contains the maximum value of $U$.
Furthermore, whenever $p$ modifies $U$ during the loop on line~\ref{ln:updatelocal}, it updates the value of $v$ so that it contains the maximum value of $U$ on lines~\ref{ln:maxval} and \ref{ln:minindex}.
This gives us the following observation.

\begin{observation}\label{obs:incleader}
	It must be the case that $U[v] \geq U[j]$ for all $j \neq v$ immediately before $p$ increments the $v$-th component of its local lap counter on line~\ref{ln:inc}.
\end{observation}


Since $p$ never decreases the values in its local lap counter, we obtain the following.

\begin{observation}\label{obs:alwaysforward}
	If process $p$ has a local lap counter $U$ in a configuration $C$ of an execution $\alpha$, and in some later configuration $C'$ of $\alpha$ it has local lap counter $U'$, then $U \preceq U'$.
\end{observation}




%\begin{observation}\label{obs:alwaysforward}
%	If process $p$ applies a \emph{Swap}$\bigl(B_i, \langle V, p\rangle\bigr)$ in some step $s$ of $\alpha$, then every \emph{Swap}$\bigl(B_{i}, \langle Y, p\rangle\bigr)$ performed by $p$ after $s$ in $\alpha$ must satisfy $V \preceq Y$.
%\end{observation}

%During the loop on line~\ref{ln:updatelocal}, $p$ updates each component $j$ of its local lap counter $U$ to be the maximum of $U'[j]$ and the current value of $U[j]$, where $U'$ is the lap counter that $p$ saw in its last swap.
%This, combined with the fact that $p$ never decreases the values in its local lap counter, gives us the following.
%
%\begin{observation}\label{obs:rememberlearn}
%	If process $p$ applies a \emph{Swap} in some step $s$ of $\alpha$ that returns a vector $V$ in the lap counter field, then every \emph{Swap}$\bigl(B_i, \langle X, p\rangle\bigr)$ operation applied by $p$ after $s$ in $\alpha$ satisfies $V \preceq X$, for every $i \in \{1, \ldots, n-1\}$.
%\end{observation}


%During the loop on line~\ref{ln:inloop}, process $p$ can only change its local lap counter on line~\ref{ln:setmaxlocal}.
%After this, $p$ restarts the loop on line~\ref{ln:inloop}.
%Hence, if $p$ swaps the base object $B_{n-1}$, then it must have been able to swap its current local lap counter into all of the base objects $B_1, \ldots, B_{n-2}$.
%This leads to the following observation.
%
%
%\begin{observation}\label{obs:swapseq}
%	If process $p$ applies a \emph{Swap}$\bigl(B_{n-1}, \langle V, p\rangle\bigr)$ in some step $s_{n-1}$ of $\alpha$, then prior to this step in $\alpha$, $p$ must have performed a sequence of steps $s_1, \ldots, s_{n-2}$, where $s_i$ is a \emph{Swap}$\bigl(B_{i}, \langle V, p\rangle\bigr)$ operation that returns $p$ in the identifier field.
%%	If process $p$ applies a Swap$\bigl(B_{n-1}, \langle V, p\rangle\bigr)$ primitive $s_{n-1}$, then prior to this, $p$ must have applied a sequence of Swap primitives $s_1, \ldots, s_{n-2}$, where $s_i$ is a Swap$(B_i, \langle V, p\rangle)$ primitive that returned $p$ in the process identifier field.
%\end{observation}



A configuration $C$ of an execution $\alpha$ is called \emph{$p$-total} in $\alpha$ if 
\begin{itemize}
\item all of $B_1, \ldots, B_{n-k}$ contain $\langle U, p\rangle$ in $C$, where $U$ is the value of $p$'s local lap counter in configuration $C$,
\item $p$ takes at least $n-k$ steps after $C$ in $\alpha$, and
\item the next $n-k$ steps by $p$ following $C$ in $\alpha$ are \emph{Swap} operations on $B_1, \ldots, B_{n-k}$ that each return $\langle
U, p\rangle$.
\end{itemize}
When $\alpha$ is clear from context, we simply say that $C$ is $p$-total.

\begin{observation}\label{obs:total}
If process $p$ applies a \emph{Swap}$(B_{n-k}, \langle U, p\rangle)$ operation in some step $s$ of an execution $\alpha$ and then either decides some value on line~\ref{ln:decide} or increments a component of its lap counter on line~\ref{ln:inc}, then there is a $p$-total configuration $C$ prior to $s$ in $\alpha$ in which $p$ has local lap counter $U$.
\end{observation}

\begin{proof}
Process $p$ only decides $v$ or completes a lap for $v$ if the condition on line~\ref{ln:conflictcond} is false.
This only occurs when each of the $n-k$ \emph{Swap} operations applied by $p$ during the loop on line~\ref{ln:swaploop} return $\langle U, p\rangle$.
Let $s'$ be the first of these $n-k$ \emph{Swap} operations, i.e. the \emph{Swap} operation applied to $B_1$.
Since $p$ is the only process that writes its identifier to any swap object, this implies that all of the swap objects contain $\langle U, p\rangle$ in the configuration that occurs immediately before $s'$.
\end{proof}

\begin{observation}\label{obs:betweentotal}
Consider some configuration $C$ that is $p$-total in an execution $\alpha$.
Suppose that there is some $p'$-total configuration $C'$ that appears after $C$ in $\alpha$.
Let $U$ and $U'$ be the local lap counters of $p$ in $C$ and $p'$ in $C'$, respectively.
If $U \not\preceq U'$, then 
\begin{enumerate}
\item there are \emph{Swap} operations $s_1, \ldots, s_{n-k}$ applied to $B_1, \ldots, B_{n-k}$ by $n-k$ distinct processes $r_1, \ldots, r_{n-k}$ different from $p'$.
These \emph{Swap} operations $s_1, \ldots, s_{n-k}$ return lap counters $U_1, \ldots, U_{n-k}$ that satisfy $U \preceq U_1, \ldots, U_{n-k}$, and
\item for all $u \in \{0, \ldots, m-1\}$ such that $U[u] > U'[u]$, there are \emph{Swap} operations $s_1, \ldots, s_{n-k}$ applied to $B_1, \ldots, B_{n-k}$ by $n-k$ distinct processes $r_1, \ldots, r_{n-k}$ different from $p'$.
These \emph{Swap} operations $s_1, \ldots, s_{n-k}$ swap lap counters $V_1, \ldots, V_{n-k}$ with $V_1[u], \ldots, V_{n-k}[u] < U[u]$ and return lap counters $U_1, \ldots, U_{n-k}$ that satisfy $U_1[u], \ldots, U_{n-k}[u] \geq U[u]$.
\end{enumerate}
\end{observation}

\begin{proof}
Notice that $p'$ is the only process that writes $p'$ to the identifier field of any object.
Hence, in configuration $C'$, $p'$ is the process that most-recently applied a swap operation to any of the objects $B_1, \ldots, B_{n-k}$.
Let $s_1', \ldots, s_{n-k}'$ be the most recent \emph{Swap} operations that $p'$ applied to $B_1, \ldots, B_{n-k}$ prior to $C'$.
Since $B_1, \ldots, B_{n-k}$ contain the lap counter $U \not\preceq U'$ in configuration $C$, all of the steps $s_1', \ldots, s_{n-k}'$ are after $C$ in $\alpha$.\todo{more detail here}
Furthermore, by Observation~\ref{} \todo{this}, each of these \emph{Swap} operations returned a lap counter $V \preceq U'$.
Then, for each $B_i$, there is a step after $C$ and before $s_i'$ in $\alpha$ in which some process swaps a lap counter $V \preceq U'$ into $B_i$.
Let $s_i$ by process $r_i$ be the first step after $C$ and before $s_i'$ in which a process swaps a lap counter $V_i$ with $U \not\preceq V_i$ into $B_i$.
Then each $s_i$ returns a lap counter $U_i$ with $U \preceq U_i$.
Thus, $p' \not\in \{r_1, \ldots, r_{n-k}\}$.
Furthermore, $r_1, \ldots, r_{n-k}$ are distinct.\todo{more detail here}
\end{proof}




%TODO

%\begin{lemma}\label{lem:allcontain}
%If process $p$ applies a \emph{Swap}$(B_{n-k}, \langle U_p, p\rangle)$ operation in some step $s_{n-k}$ of $\alpha$ and then either decides some value $v$ on line~\ref{ln:decide} or increments the $v$-th component of its lap counter on line~\ref{ln:inc}, then
%\begin{itemize}
%\item prior to $s_{n-k}$ in $\alpha$, process $p$ performed a sequence of steps $s_1, \ldots, s_{n-k-1}$, where each $s_i$ is a \emph{Swap}$(B_i, \langle U_p, p\rangle)$ operation,
%\item for all $1 \leq i \leq n-k$, the step $s_i$ returns $\langle U_p, p\rangle$, and
%\item in the configuration $C$ that immediately precedes step $s_1$ in $\alpha$, the objects $B_1, \ldots, B_{n-k}$ contain the value $\langle U_p, p\rangle$.
%\end{itemize}
%\end{lemma}
%
%\begin{proof}
%Process $p$ only decides $v$ or completes a lap for $v$ if the condition on line~\ref{ln:conflictcond} is false.
%This only occurs when each of the \emph{Swap} operations applied by $p$ during the loop on line~\ref{ln:swaploop} return $\langle U_p, p\rangle$.
%Since $p$ is the only process that writes its identifier to any swap object, this implies that all of the swap objects contain $\langle U_p, p\rangle$ in the configuration that occurs immediately before $s_1$.
%\end{proof}

\begin{lemma}\label{lem:agree}
Algorithm~\ref{alg:consswap} satisfies agreement.
\end{lemma}

\begin{proof}
Consider some execution $\alpha$ of the algorithm in which exactly $k$ distinct values $v_1, \ldots, v_k$ are decided.
We show that, for any extension $\alpha'$ of $\alpha$, any process that decides during $\alpha'$ decides some value in $\{v_1, \ldots, v_k\}$.
For all $i \in \{1, \ldots, k\}$, let $p_i$ be a process that decides $v_i$ during $\alpha$.
By Observation~\ref{obs:total}, there is a $p_i$-total configuration $C_i$ before the step in which $p_i$ decides.
%By Lemma~\ref{lem:allcontain}, $p_i$ performs the sequence of steps $s_{i,1}, \ldots, s_{i,n-k}$ and then decides $v_i$, where each step $s_{i,j}$ is a \emph{Swap}$(B_j, \langle U_{p_i}, p_i\rangle)$ that returns $\langle U_{p_i}, p_i\rangle$.
%Furthermore, in the configuration $C_i$ that immediately precedes $s_{i,1}$, every object $B_1, \ldots, B_{n-k}$ contains the value $\langle U_{p_i}, p_i\rangle$.
Without loss of generality, suppose that $C_1, \ldots, C_k$ appear in order during $\alpha$.
For all $i$, let $U_i$ be the local lap counter of $p_i$ in $C_i$.
Define $\ell_i = U_{i}[v_i]$ for all $i$.


Suppose that in configuration $C_k$, every undecided process $q$ either has a preference $u$ and local lap counter $V$ with $V[u] < \ell_k$, or $u \in \{v_1, \ldots, v_k\}$.
Then every process that decides in any extension $\alpha'$ of $\alpha$ decides some value in $\{v_1, \ldots, v_k\}$. \todo{prove this}
This completes the proof of agreement.


Otherwise, some process $q$ has a local lap counter $V$ and preference $u$ in configuration $C_k$, where $u \not\in \{v_1, \ldots, v_k\}$ and $V[u] \geq \ell_k$.
Let $L = V[u]$.
Since $\ell_k \geq 2$ by Observation~\ref{} \todo{this}, $L \geq 2$.
By Observation~\ref{} \todo{this}, prior to configuration $C_k$ in $\alpha$, some process $r$ takes a step in which it increases the $u$-th component of its local lap counter from $L - 1$ to $L$.
Let $V'$ be the local lap counter of process $r$ immediately before this step.
Then $V'[u] = L-1$.
By Observation~\ref{obs:total}, there is an $r$-total configuration $C$ prior to this step in which $r$ has the local lap counter $V'$.


Since $p_k$ decides $v_k$ in the step $s_{k, n-k}$, we know that $\ell_k \geq U_{p_k}[u] + 2$ by the condition on line~\ref{ln:decidecond}.
Hence, by Observation~\ref{obs:betweentotal}, $n-k$ distinct processes $r_1, \ldots, r_{n-k}$ different from $p_k$ swap lap counters whose $u$-th components are at most $\ell_k - 2$ to $B_1, \ldots, B_k$ between $C$ and $C_k$ in $\alpha$, and the $u$-th component of the lap counters in the responses to these swap operations are at least $L-1$.
Following these swap operations by $r_1, \ldots, r_{n-k}$, these processes update the $u$-th component of their local lap counters to a value that is at least $L-1$ in the loop on line~\ref{ln:updatelocal}.
By Observation~\ref{}, process $r$ can only swap lap counters whose $u$-th components are at least $L$ after $C$.
Hence, $r \not\in \{r_1, \ldots, r_{n-k}\}$.
%So $|\{q'\} \cup \{r_0, \ldots, r_{n-k-1}\}| = n-k+1$, $|\{p_1, \ldots, p_{k-1}\}| = k-1$, and none of these processes are $p_k$.
Thus, at least one of $r, r_1, \ldots, r_{n-k}$ is in $\{p_1, \ldots, p_{k-1}\}$.
Hence, there is at least one $p_j \in \{p_1, \ldots, p_{k-1}\}$ with $U_{p_j}[u] \geq L-1$.
Let $j$ be the maximum number for which this is satisfied.

Since $p_j$ decides $v_j$, we know that $U_{p_j}[v_j] \geq U_{p_j}[u] + 2 \geq L+1$.
Furthermore, $U_{p_k}[v_k] = \ell_k \geq U_{p_k}[v_j] + 2$.
By Observation~\ref{} \todo{this}, $n-k$ distinct processes $r_1', \ldots, r_{n-k}'$ different from $p_k$ swap $B_1, \ldots, B_k$ between $C_j$ and $C_k$ in $\alpha$, and the lap counters in the responses to these operations are $\succeq U_{p_j}$.
If there is a process $p_{m} \in \{r_1', \ldots, r_{n-k}'\}$, then $U_{p_{m}} \succeq U_{p_j}$.
Hence, $U_{p_m}[u] \geq U_{p_j}[u] \geq L$.
Furthermore, $m > j$ since $p_1, \ldots, p_{j-1}$ terminated before $C_j$ in $\alpha$.
But this contradicts the definition of $j$.
Hence, $p_1, \ldots, p_k \not\in \{r_1', \ldots, r_{n-k}'\}$.
If $r \in \{r_1', \ldots, r_{n-k}'\}$, then $U_r \succeq U_{p_j}$.
Then $U_r[v_j] \geq U_{p_j}[v_j] \geq L+1$.
This means that $r$ cannot have preference $u$ in $C_k$, which is a contradiction.
\end{proof}





\begin{lemma}\label{lem:onebyone}
	Suppose some process $p$ applies a \emph{Swap}$\bigl(B_{n-1}, \langle V, p\rangle\bigr)$ operation in some step $s$ of $\alpha$, where $V[v] > 1$ for some $v \in \{0, \ldots, m-1\}$.
	Then, for all $c \in \{2, \ldots, V[v]\}$, there must be some step before $s$ in $\alpha$ by some process $q$ such that, at the end of the step $s$, $q$ increments the $v$-th component of its local lap counter on line~\ref{ln:inc} from $c-1$ to $c$.
\end{lemma}

\begin{proof}
Let $c \in \{2, \ldots, V[v]\}$.
Let $s'$ be the first step in $\alpha$ such that, at the end of the step $s'$, the process $q$ that applied $s'$ updates its local lap counter $U_q$ so that $U_q[v] \geq c$.
Notice that $p$'s local lap counter $U_p$ satisfies $U_p[v] = V[v] \geq c$ immediately before the step $s$.
Hence, $s'$ happens before $s$ in $\alpha$.

At the end of the step $s'$, process $q$ either updates its local lap counter so that $U_q[v] \geq c$ in the loop on line~\ref{ln:updatelocal} or on line~\ref{ln:inc}.
If $q$ updates its local lap counter in the loop on line~\ref{ln:updatelocal}, this implies that the response to $s'$ contained a lap counter $U'$ such that $U'[v] \geq c$.
Suppose that the \emph{Swap} operation in $s'$ is applied to the object $B_i$ and $q'$ was the process that last swapped the lap counter $U'$ into $B_i$ prior to $s'$.
Then the local lap counter of $q'$ must have been equal to $U'$ prior to $s'$.
Hence, at the end of some step before $s'$, process $q'$ changes the $v$-th component of its local lap counter to $U'[v] \geq c$.
This contradicts the definition of $s'$.

Therefore, $q$ must have updated its local lap counter on line~\ref{ln:inc}.
By inspection of the code, this means that $q$ incremented the $v$-th component of its local lap counter from $c-1$ to $c$.
\end{proof}





\begin{lemma}\label{lem:valid}
Algorithm~\ref{alg:consswap} satisfies validity.
\end{lemma}

\begin{proof}
Consider an execution $\alpha$ of Algorithm~\ref{alg:consswap} in which some process $p$ decides a value $v$.
We need to prove that some process had input $v$.
No process ever decreases the value of any component of its local lap counter, so every component of every process' lap counter is always nonnegative.
Hence, the condition on line~\ref{ln:decidecond} implies that the $v$-th component of $p$'s local lap counter is at least $2$ when $p$ decides.
Let $s$ be the first step in $\alpha$ in which some process $q$ changes the $v$-th component of its local lap counter so that it is greater than $0$.
Then $q$ changes the $v$-th component of its local lap counter at the end of step $s$ on line~\ref{ln:init2}, line~\ref{ln:setmaxlocal}, or line~\ref{ln:inc}.

If $q$ changes the $v$-th component of its local lap counter on line~\ref{ln:init2}, then $q$ had input $v$.
This completes the proof of the lemma.

We now show that both other cases lead to a contradiction.
First, suppose $q$ changes the $v$-th component of its local lap counter at the end of $s$ on line~\ref{ln:setmaxlocal}.
Then the response of the \emph{Swap} operation that $q$ performed on line~\ref{ln:swap} during $s$ must have held a lap counter $U'$ with $U'[v] > 0$.
Hence, prior to $s$, the local lap counter of some process was equal to $U'$.
This contradicts the definition of $s$.

Now suppose $q$ changes the $v$-th component of its local lap counter at the end of $s$ on line~\ref{ln:inc}.
Then $q$ changes the $v$-th component of its local lap counter from $0$ to $1$ during $s$.
Observation~\ref{obs:incleader} implies that all of the other components of $q$'s local lap counter are $0$ during $s$.
However, on line~\ref{ln:init2}, $q$ sets some component of its local lap counter to $1$, and it never decreases the value of any component of its local lap counter.
This is a contradiction.
\end{proof}

\begin{lemma}\label{lem:of}
Algorithm~\ref{alg:consswap} is obstruction-free.
\end{lemma}

\begin{proof}
We argue that, for any configuration $C$ of Algorithm~\ref{alg:consswap}, the solo-terminating execution by $p$ from $C$ applies at most $\frac{n(n-1)}{2} + 2(n-1)$ \emph{Swap} operations.
First notice that process $p$ only restarts the loop on line~\ref{ln:inloop} by resetting $i$ to $1$ if the condition on line~\ref{ln:idcond} holds.
This condition is met only if the previous \emph{Swap} operation applied by $p$ on line~\ref{ln:swap} returned a process identifier different from $p$.
This happens at most once for each base object in $p$'s solo-terminating execution, so $p$ restarts the loop on line~\ref{ln:inloop} at most $n-1$ times.
If $p$ restarts this loop $n-1$ times, it applies at most $\frac{n(n-1)}{2}$ \emph{Swap} operations during this execution.

Let $v$ be the value of $p$'s preference once every base object contains $p$ in its identifier field.
Then $p$ increments $U[v]$ on line~\ref{ln:inc} at most twice before the condition on line~\ref{ln:decidecond} is satisfied.
Process $p$ performs at most $n-1$ \emph{Swap} operations during any iteration of the loop on line~\ref{ln:mainloop} if every base object contains $p$ in the identifier field throughout the iteration.
Hence, $p$ applies at most $2(n-1)$ more \emph{Swap} operations.
In total, $p$ applies at most $\frac{n(n-1)}{2} + 2(n-1)$ \emph{Swap} operations during its solo-terminating execution from $C$.
Therefore, Algorithm~\ref{alg:consswap} is obstruction-free.
\end{proof}

Lemmas~\ref{lem:agree}-\ref{lem:of} imply that Algorithm~\ref{alg:consswap} is an $n$-process, $m$-valued, obstruction-free consensus algorithm.




\section{Lower Bound on Set Agreement from Swap}\label{sec:unreadablelb}




We now present our lower bound on the number of swap objects required to solve nondeterministic solo-terminating, $(k+1)$-valued, \todo{decide whether to use commas or not} $k$-set agreement.
Consider an initial configuration $C$ and an execution $\alpha$ from $C$ in which $k$ distinct values are decided.
Let $\mathcal{Q}$ be a set of processes that do not participate in $\alpha$, and suppose that in $C$ the processes in $\mathcal{Q}$ have input $v$, which is different from all of the values decided in $C\alpha$.
%In the following lemma, we show that in the configuration $C\alpha$, at least $|\mathcal{Q}|$ swap object must contain information about the execution $\alpha$.
If a process $q \in \mathcal{Q}$ starts running in $C\alpha$, then it cannot tell that $k$ different values have been decided until it applies a \emph{Swap} operation to some object that was modified during $\alpha$.
However, when $q$ first swaps some object $B$ that was modified during $\alpha$, process $q$ overwrites the information about $\alpha$ that was stored there.
Hence, if we stop $q$ immediately after it swaps $B$, no other process in $\mathcal{Q}$ can learn anything about $\alpha$ by swapping $B$.
We apply this argument repeatedly, using processes to overwrite the objects that store information about $\alpha$ one at a time.
This shows that $\alpha$ must have swapped at least $|\mathcal{Q}|$ different objects.
We formalize this argument in the proof of Lemma~\ref{lem:consume}.



\begin{lemma}\label{lem:consume}
	Consider an initial configuration $C$ of a nondeterministic solo-terminating $k$-set agreement algorithm in which a set of processes $\mathcal{Q}$ have the same input $v$.
	Let $\alpha$ be an execution from $C$ that contains no steps by processes in $\mathcal{Q}$ such that $k$ distinct values different from $v$ are decided in $C\alpha$.
	Then $\alpha$ accesses at least $|\mathcal{Q}|$ swap objects.
\end{lemma}

\begin{proof}
Let $\mathcal{Q} = \{q_1, \ldots, q_{|\mathcal{Q}|}\}$.
Define $\mathcal{Q}_i = \{q_1, \ldots, q_i\}$ for all $i \in \{1, \ldots, |\mathcal{Q}|\}$, and define $\mathcal{Q}_0 = \emptyset$.
Let $D$ be an initial configuration in which all processes have input $v$.
For all $0 \leq i \leq |\mathcal{Q}|$, we show that there is a set of $i$ objects $\mathcal{B}_i \subseteq \mathcal{B}$ and a pair of $\mathcal{Q}_i$-only executions $\gamma_i$ and $\delta_i$ from $C\alpha$ and $D$, respectively, such that $\textit{value}(B, C\alpha) = \textit{value}(B, D)$, for all $B \in \mathcal{B}_i$.
We use induction on $i$.
When $i = 0$, $\gamma_i$ and $\delta_i$ are empty executions, $\mathcal{B}_i = \emptyset$, and the claim is trivially satisfied.

Now suppose the claim holds for some $i \in \{0, \ldots, |\mathcal{B}|-1\}$.
Notice that $C\alpha\gamma_i \widesim{q_{i+1}} D\delta_i$, since $q_{i+1}$ has input $v$ in both configurations and takes no steps in $\alpha$, $\gamma_i$, or $\delta_i$.
Consider a $q_{i+1}$-only solo-terminating execution $\sigma$ from $D\delta_i$.
By validity, $q_{i+1}$ decides $v$ in $\sigma$.
Let $\tau$ be the longest prefix of $\sigma$ such that $q_{i+1}$ only accesses objects in $\mathcal{B}_i$ during $\tau$.
By the induction hypothesis, $\textit{value}(B, C\alpha\gamma_i) = \textit{value}(B, D\delta_i)$ for all $B \in \mathcal{B}_i$.
Hence, there is a $q_{i+1}$-only execution $\tau'$ from $C\alpha\gamma_i$ such that $\tau \widesim{q_{i+1}} \tau'$.
If $\tau = \sigma$, then $q_{i+1}$ decides $v$ in $\tau$ and $\tau'$.
This contradicts agreement, since $k$ distinct values different from $v$ are decided in $C\alpha$.
Thus, $\tau$ is a proper prefix of $\sigma$.

Let $s$ and $s'$ be the step that $q_{i+1}$ is poised to apply in $D\delta_i\tau$ and $C\alpha\gamma_i\tau'$, respectively.
Since $C\alpha\gamma_i \widesim{q_{i+1}} D\delta_i$ and $\tau' \widesim{q_{i+1}} \tau$, we have $C\alpha\gamma_i\tau' \widesim{q_{i+1}} D\delta_i\tau$.
Thus, $s$ and $s'$ are the same \emph{Swap} operation by $q_{i+1}$.
By definition of \emph{Swap}, if $B^\star$ is the object accessed by $s$ and $s'$, then $\textit{value}(B^\star, C\alpha\gamma_i\tau's') = \textit{value}(B^\star, D\delta_i\tau s)$.
Furthermore, by definition of $\tau$, we know that $B^\star \not\in \mathcal{B}_i$.
Hence, taking $\gamma_{i+1} = \gamma_i\tau's'$, $\delta_{i+1} = \delta_i\tau s$, and $\mathcal{B}_{i+1} = \mathcal{B}_i \cup \{B^\star\}$ completes the inductive step.

Taking $i = |\mathcal{Q}|$ gives us a set of $|\mathcal{Q}|$ objects $\mathcal{B}_{|\mathcal{Q}|}$.
This completes the proof of the lemma.
\end{proof}



\begin{theorem}\label{thm:swaplb}
%	Suppose that $\mathcal{B}$ is a set of base objects with unbounded domain size that support only the \emph{Swap} operation.
	For all $n > k \geq 1$, every nondeterministic solo-terminating, $n$-process, $(k+1)$-valued, $k$-set agreement algorithm from swap objects uses at least $\lceil\frac{n}{k}\rceil - 1$ objects.
\end{theorem}

\begin{proof}
	Consider such an algorithm for the set of processes $\mathcal{P} = \{p_0, \ldots, p_{n-1}\}$.
	We will use induction on $k$.
	When $k = 1$, consider an initial configuration $C$ of the algorithm in which process $p_0$ has input $0$ and all other processes have input $1$.
	Let $C_0$ be an initial configuration in which all processes have input $0$.
	Let $\alpha$ be a solo-terminating execution by $p_0$ from $C$.
	Since $C_0 \widesim{p_0} C$ and all of the base objects have the same values in $C_0$ and $C$, there is a $p_0$-only execution $\alpha'$ by $p_0$ from $C_0$ such that $\alpha' \widesim{p_0} \alpha$.
	Since $p_0$ decides during $\alpha$, it must decide during $\alpha'$ as well.
	By validity, $p_0$ decides $0$ during $\alpha'$, which implies that $p_0$ decides $0$ during $\alpha$.
	Lemma~\ref{lem:consume} (with $\mathcal{Q} = \{p_1, \ldots, p_{n-1}\}$ and $v = 1$) implies that $\alpha$ accesses at least $n-1$ swap objects, which completes the proof of the base case.
	
	Now let $1 < k < n$ and suppose the theorem holds for $k-1$.
	Let $\mathcal{R}$ be the first $\bigl\lceil \frac{n(k-1))}{k}\bigr\rceil$ processes in $\mathcal{P}$.
	Let $\mathcal{I}$ be the set of all initial configurations in which $\mathcal{R}$'s inputs are in $\{0, \ldots, k-1\}$.
	If, for every initial configuration $C \in \mathcal{I}$ and every $\mathcal{R}$-only execution from $C$, at most $k-1$ different values are decided in $\alpha$, then the algorithm solves nondeterministic solo-terminating, $k$-valued, $(k-1)$-set agreement among the processes in $\mathcal{R}$.
	Hence, by the induction hypothesis, the algorithm uses at least $\frac{1}{k-1}\cdot \bigl\lceil\frac{n(k-1)}{k}\bigr\rceil - 1 = \lceil\frac{n}{k}\rceil - 1$ swap objects.
	
	Otherwise, there is an initial configuration $C \in \mathcal{I}$ and a $\mathcal{R}$-only execution $\alpha$ from $C$ in which all $k$ values $0, \ldots, k-1$ are decided.
	Notice that $|\mathcal{P} - \mathcal{R}| = n - \bigl\lceil\frac{n(k-1)}{k}\bigr\rceil = \lfloor\frac{n}{k}\rfloor \geq \lceil\frac{n}{k}\rceil - 1$.
	Hence, by Lemma~\ref{lem:consume} (with $\mathcal{Q} = \mathcal{P} - \mathcal{R}$ and $v = k$), $\alpha$ accesses at least $\mathcal{P} - \mathcal{R} \geq \lceil\frac{n}{k}\rceil - 1$ swap objects.
	This completes the proof of the theorem.
\end{proof}


Theorem~\ref{thm:swaplb} implies that nontrivial operations alone cannot be used to solve nondeterministic solo-terminating $k$-set agreement with fewer than $\lceil\frac{n}{k}\rceil-1$ historyless objects.
The proof of Lemma~\ref{lem:consume} exploits a key limitation of nontrivial operations on historyless objects.
In order to learn important information stored in a historyless object that only supports nontrivial operations, a process must overwrite that information.
This prevents other processes from learning the information.
The reason this argument does not work with readable swap objects is because, by using a \emph{Read} operation, a process in $\{p_1, \ldots, p_{n-1}\}$ can see that $p_0$ decided $0$ without overwriting any of the information that $p_0$ wrote.

%Ellen, Gelashvili, and Zhu \citep{egz-18} proved that space lower bounds for obstruction-free consensus algorithms also hold for nondeterministic solo-terminating (and hence, randomized wait-free) consensus algorithms.
%Combined with Theorem~\ref{thm:swaplb}, this gives us the following.

Since all obstruction-free and randomized wait-free consensus algorithms are also nondeterministic solo-terminating, Theorem~\ref{thm:swaplb} gives us the following.

\begin{corollary}
	For all $n > k \geq 1$, every obstruction-free or randomized wait-free, $n$-process, $(k+1)$-valued, $k$-set agreement algorithm from swap objects requires at least $\lceil\frac{n}{k}\rceil - 1$ objects.
\end{corollary}
